Reference-Steering via Data-Driven Predictive Control for Hyper-Accurate Robotic Flying-Hopping Locomotion

State-of-the-art model-based control designs have been shown to be successful in realizing dynamic locomotion behaviors for robotic systems. The precision of the realized behaviors in terms of locomotion performance via fly, hopping, or walking has not yet been well investigated, despite the fact that the difference between the robot model and physical hardware is doomed to produce inaccurate trajectory tracking. To address this inaccuracy, we propose a referencing-steering method to bridge the model-to-real gap by establishing a data-driven input-output (DD-IO) model on top of the existing model-based design. The DD-IO model takes the reference tracking trajectories as the input and the realized tracking trajectory as the output. By utilizing data-driven predictive control, we steer the reference input trajectories online so that the realized output ones match the actual desired ones. We demonstrate our method on the robot PogoX to realize hyper-accurate hopping and flying behaviors in both simulation and hardware. This data-driven reference-steering approach is straightforward to apply to general robotic systems for performance improvement via hyper-accurate trajectory tracking.

==> notes/DeepcNotes.tex <==
\section{Notes from Course}

\begin{definition}
    Let $u:\mathbb{Z}\rightarrow \mathbb{R}^m$, and $t_0,t_1 \in \mathbb{Z}_{\geq 0}, t_0 \leq t_1$, the sequence $u_{t_0,t_1}$ is \textbf{persistently exciting}  of L if $\mathcal{H}_L(u_{t_0,t_1})$ has full row rank.
\end{definition}

Consider LTI system:
$$
\left\{
\begin{aligned}
 x_{k+1}& = Ax_{k} + Bu_{k}\\
 y_{k} &= Cx_{k} + Du_{k}    
\end{aligned}\quad\text{(*)}
\right.
$$
The model (*)

$$
y_{[0,L]} = \mathcal{O}_L x_0 + \mathcal{T} u_{[0,L]}
$$

$$
\left[\begin{matrix}
    y_{(0)}\\    y_{(1)}\\    \vdots\\    y_{(L-1)}
\end{matrix}\right]=
\left[\begin{matrix}
    C\\    CA\\    \vdots\\    CA^{L-1}
\end{matrix}\right]x_0+
\left[\begin{matrix}
    D & 0 & \cdots   &  0\\
    CB & D & \cdots  &  0\\
    CAB & CB & D &  0\\
    \vdots\\
    CA^{L-1}B & \cdots &&D\\
\end{matrix}\right]
\left[\begin{matrix}
    u_{(0)}\\    u_{(1)}\\    \vdots\\   u_{(L-1)}
\end{matrix}\right]
$$


==> notes/MotorExample.tex <==
\section{Motor Example}
Here we have a simple casade control of a DC motor, consisting of a PD motion controller and a P current controller, we take $\theta$, $\dot\theta$, and current $I$ as the state variable and use PD control to generate a desired current, the inner loop of the control system is using proportional(P) control for Current, integration will be a little bit difficult. The $PI$ format is :$V = K_{p2}(I-I_d) + \int K_{I2}(I-I_d)dt )$
The pendulum dynamics and the motor dynamics:
\begin{equation}
\begin{aligned}
mR^2\ddot\theta &= -b\dot\theta + k_tI_a & \text{(system dynamics)}\\
I_d &= K_p(\theta_d-\theta) + K_d (\dot\theta_d - \dot\theta ) & \text{(PD control)} \\
V &= K_{p2}(I_d-I_a) & \text{(P control)} \\
V &= k_e n\dot\theta + I^a R + L\dot{I_a} & \text{(motor dynamics)} \\
\end{aligned}
\end{equation}



Take these as state variables, $I_a, \theta, \dot\theta$, we have the state space equations:
\begin{equation}
\begin{aligned}
\dot \theta&  = \dot \theta\\
\ddot \theta& = \frac{-b}{mR^2}\dot\theta + \frac{k_t}{mR^2} I_a\\
\dot I_a& =  -(K_{p2}+R)/L\cdot I_a - (k_en+K_{p2}K_d)/L\dot\theta -K_{p2}K_p/L\theta\\
& \ + K_{p2}K_p/L\theta_d + K_{p2}K_{d}/L\dot\theta_d
\end{aligned}
\end{equation}
Next, take $\theta_d, \dot\theta_d$ as system input and write it down as state-space format of control system: 
\begin{equation}
\begin{aligned}
\left[
\begin{matrix}
\dot\theta\\
\ddot\theta\\
\dot{I_a}
\end{matrix}
\right]
&=
\left[
\begin{matrix}
0 & 1 & 0\\
0 & \frac{-b}{mR^2} & \frac{k_t}{mR^2}\\
-K_{p2}K_p/L & -(k_en+K_{p2}K_d)/L & -(K_{p2}+R)/L
\end{matrix}
\right]
\left[
\begin{matrix}
\theta\\
\dot\theta\\
{I_a}
\end{matrix}
\right]
+ \\
& \quad
\left[
\begin{matrix}
0&0\\
0&0\\
K_{p2}K_p/L & K_{p2}K_{d}/L\\
\end{matrix}
\right]
\left[
\begin{matrix}
\theta_d\\
\dot\theta_d
\end{matrix}
\right]
\end{aligned}
\end{equation}

\begin{equation}
    \begin{aligned}
        y = C x = \left[\begin{matrix}
    1 & 0 & 0\\ 0 & 1 & 0\\
\end{matrix}\right] x =\left[ \begin{matrix}
            \theta\\ \dot \theta 
        \end{matrix}\right]
    \end{aligned}
\end{equation}

To test DeePC, we used several controllers to compare their control quality, we don't want to use these controllers to take account of current directly (taking y as the state instead).\\

\textbf{State Feedback controller}: Using LQR to calculate controller gain, with Q = diag(1e2, 2e1, 0). R = diag(0.1, 0.1) We don't want to penalize our control input too much.
K = LQR(A,B,Q,R).

\textbf{MPC controller}: horizon = 10 similar feedback controller as

\textbf{DeePC controller}: $T_{ini}=25$, $T_{ftr}=10$, taking a time series of 100Hz, 0.5s to build Hankel matrix. $\lambda_u=[0.1,0.1],\ \lambda_y=[1e6,1e2],\ \lambda_g=2e2,\ \lambda_{ini}=1e6$.

==> notes/ToDo.tex <==
\section{ToDo}
%%% Introduction
1. Compare with other Open source platforms 
\href{https://github.com/DRCL-USC/Hector_Simulation}{USC Biped}\\
(compare: hardware is not open-sourced\\
(inspiration: system and control architecture can mimic its figure \\
\href{https://github.com/RoboDesignLab/HOPPY-Project}{HOPPY jumping robot}\\
(compare: not a real bipedal robot, cannot be algorithm test bed\\
(inspiration:\\
\href{https://open-dynamic-robot-initiative.github.io/}{NYU dynamic robot initiative} \\
(compare:  4000 dollars, pure-3D printed, small load capacity, not so durable\\
(inspiration: choose open source protocol, learning its introduction writing method\\
\href{https://www.opensourceleg.org/about}{Umich open sourced leg}
(compare: \\
(inspiration: \\
Oncilla 
\href{https://ieeexplore.ieee.org/document/8794436/authors#authors}{Stanford-doggo}

\textbf{
1. Find all the papers or repos contain open-sourced robotic platforms.(\checkmark)\\
\indent 2. Compare and find our advantages.()\\
}

%%% Advantages
1. Low cost\\
2. versatile(education toolkit, research platform)\\
3. 2D -> for thoroughly evaluated algorithms, state of the art software architecture, \\
3. terrain(cheap \& versatile) and propeller(quantitative disturbance), modular system for other things. Design optimization. Off the shelf parts: no machining, but still durable. Customize repurpose the configuration or functionality of the robot.  \\
\textbf{1. Write out the mechanical design, electronics and software part of the paper(\checkmark)
2. Write out HLIP theory part of the paper
3. Write out Adaptive HLIP theory part of the paper 
4. Write out the introduction ()}


%%% Open Source Repo 
Open source: 
Mechanical design: BOM, CAD drawing,
Electrical: Wiring diagram
C++ repo, MATLAB simulator, 

%%% Experiments
\subsection{Experiments}

1. Rigid flat ground and step in place(if possible), velocity tracking

2. Terrain adaptation ( steady velocity on all granular terrains )

3. External disturbance (test the propeller(\checkmark))

4. design optimization (change leg inertia, leg length (both shin and thigh))


\begin{table}
    \centering
    \begin{tabular}{c|c|c|c}
       Category &  \\\hline 
       flat ground walking(velocity)  & 0.0m/s &  & \\\hline
       terrain adaptation  &  &  & \\\hline
       disturbance rejection  & 10N-h & 10N-v & 10N-(h+v)\\\hline
       design optimization  & 150 &  & \\\hline
    \end{tabular}
    \caption{Caption}
    \label{}
\end{table}

%%%% Detailed todo list
\textbf{\\
1. Design a new cover to cover all the wires(\checkmark)\\
2. A new more curved and wide contact foot(\checkmark)\\
3. Clean up the wire configuration for the boom and setup experiment place in the middle()\\
4. Renew step planning for legs.(\checkmark)\\
5. Test 4. in simulator(\checkmark)\\
6. Modify and print a new version of the foot, tire textures(\checkmark)\\
7. Add logic so robot will return to initial configuration after hanging in air.(\checkmark)}
\\



==> notes/old_method.tex <==

\section{Methods}

In this section, we introduce the framework of data driven output-steering, and the specifications of how to perform this framework on robotics systems, to tackle noise in reading, to use this when there are dynamics, and possible non-linearity of the input-output dynamics.

\subsection{Output Steering}
% Assume the system has linear hidden dynamics and is not perfect.
% A picture showing the output steering framework
% One key feature of output-steering is that, when you have no authority to lower level controller, or there are unmodelled dynamics, you are able to use data to re-target and improve the performance of the controller, without accessing the inner loop.

\subsection{Noise Robust PEM-MPC Formulation}
% DeePC -> PEM-MPC with slack
The aforementioned DeePC formulation suffers from computational issues since the problem size is directly related to number of data used.  
In \cite{DeePC_fist_paper}, 
To accelerate computation: PEM-MPC \cite{PEM-MPC_quadruped}\cite{PEM-MPC_origin}. And method to offline calculate a prediction matrix is introduced without loss of information of the original Hankel matrix.
For the uniqueness of solution, and the ability to avoid noise
To deal with robustness problem: Adding slack variable\\
To address discontinuous dynamics: trajectory-filling.

% output steering 


\subsection{DeePC for Hybrid Dynamical Systems}
% fake trajectory design
% Reference Steering for Hybrid Locomotion 
% One major issue for genear, which lost 
One key factor that would cause is that, when the system ,which is very oftenly seen in legged robots, the dyanamics
The formulation of the trajectory filling would then be: 

with 
\begin{equation}
\begin{aligned}
\min_{u_{gini}, y_{gini}, g}& ||g||^2+||u||^2_{\Sigma}+||y||^2_{\Sigma}  \\
\text{s.t.}\quad& H_Gg=\begin{bmatrix}u_{pre}\\ u_{g} \\ u_{f} \\ y_{pre}\\ y_{g}\\y_{f}\end{bmatrix}  \\
&u\in\mathcal{U} \\
&y\in\mathcal{Y}
\end{aligned}
\end{equation}
Using the trajectory that can the flying phase to fill in the trajectory of the , we obtain the data to 

\subsection{Control Method forming on PogoX}
Fix energy level trajectory following.


